A Dense Tensor Accelerator with Data Exchange Mesh for DNN and Vision Workloads

We propose a dense tensor accelerator called VectorMesh, a scalable, memory-efficient architecture that can support a wide variety of DNN and computer vision workloads. Its building block is a tile execution unit~(TEU), which includes dozens of processing elements~(PEs) and SRAM buffers connected through a butterfly network. A mesh of FIFOs between the TEUs facilitates data exchange between tiles and promote local data to global visibility. Our design performs better according to the roofline model for CNN, GEMM, and spatial matching algorithms compared to state-of-the-art architectures. It can reduce global buffer and DRAM fetches by 2-22 times and up to 5 times, respectively.

==> 20_related.tex <==
\section{Related Works}

==> large_float/table_area.tex <==
\begin{table}[ht]
\centering
\small
\caption{Area estimation of the architectures, based on synthesized statistics from Eyeriss.}\label{tab:area_norm}
\begin{tabular}{lrrr}
\toprule
                & Eyeriss & TPU & VectorMesh\\
\midrule
MAC             & 0.08 & 0.08 & 0.08\\
Global buffer   & 0.19 & 0.38 & 0.00\\
Local buffer    & 0.48 & 0.00 & 0.67\\
Controllers     & 0.25 & 0.00 & 0.25\\
BFN+FIFO        & 0.00 & 0.00 & 0.04\\
\hline
Area factor ($A$) & 1.00 & 0.46 & 1.04\\
\bottomrule
\end{tabular}
\end{table}
